Complex Structure in Class 0 Protostellar Envelopes III: Velocity Gradients in Non-Axisymmetric Envelopes, Infall or Rotation?

We present an interferometric kinematic study of morphologically complex protostellar envelopes based on observations of the dense gas tracers N2H+ and NH3. The strong asymmetric nature of most envelopes in our sample leads us to question the common interpretation of velocity gradients as rotation, given the possibility of projection effects in the observed velocities. Several "idealized" sources with well-ordered velocity fields and envelope structures are now analyzed in more detail. We compare the interferometric data to position-velocity diagrams of kinematic models for spherical rotating collapse and filamentary rotating collapse. For this purpose, we developed a filamentary parametrization of the rotating collapse model to explore the effects of geometric projection on the observed velocity structures. We find that most envelopes in our sample have PV structures that can be reproduced by an infalling filamentary envelope projected at different angles within the plane of the sky. The infalling filament produces velocity shifts across the envelope that can mimic rotation, especially when viewed at single-dish resolutions and the axisymmetric rotating collapse model does not uniquely describe any dataset. Furthermore, if the velocities are assumed to reflect rotation, then the inferred centrifugal radii are quite large in most cases, indicating significant fragmentation potential or more likely another component to the line-center velocity. We conclude that ordered velocity gradients cannot be interpreted as rotation alone when envelopes are non-axisymmetric and that projected infall velocities likely dominate the velocity field on scales larger than 1000 AU.

==> tab3.tex <==
\begin{deluxetable}{lllllll}

\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Source Properties}
\tablehead{
  \colhead{Source} & \colhead{Distance}  & \colhead{Gradient PA} & \colhead{$R_{SS}$} & \colhead{$R_C$(9000)} & \colhead{$R_C$($R_{SS}$)} & \colhead{Gradient (9000AU)}\\
                    & \colhead{(pc)}     & \colhead{($^{\circ}$)}& \colhead{(AU)}     & \colhead{(AU)}        & \colhead{(AU)}            & \colhead{(km s$^{-1}$ pc$^{-1}$)} \\

}
\startdata
IRAS 03282+3035    & 300 &  -      & -    & -     &  -   & -   \\
HH211-mm           & 300 &  29     & 1000?& 7100  &  2   & 12.83\\
L1521F             & 140 &  0      & -    & 20    &  -   & 0.68\\
IRAS 04325+2402    & 140 &  90     & -    & -     &  -   & 6.89\tablenotemark{a}\\
L1527              & 140 &  0      & 1120 & 1600  &  11  & 6.01\\
RNO43              & 420 &  110    & 1800 & 1500  &  230 & 5.84\\
HH270 VLA1         & 420 &  -      & -    & -     &  -   & -   \\
IRAS 16253-2429    & 125 &  108    & 1300 &  3    &  -   & 0.62\\
L483               & 200 &  15     & -    & 2150  &  -   & 7.05\\
Serpens MMS3       & 300 &  60     & 1800 & 430   &  85  & 3.15\\
HH108IRS           & 300 &  118    & 1950 & 140   &  43  & 1.8 \\
L673-SMM2          & 300 &  -      & -    & -     &  -   & -   \\
L1152              & 300 &  135    & -    & -     &  -   & 3.27\tablenotemark{a}\\
L1157              & 300 &  70     & 1350 & 150   &  14  & 1.86\\
CB230              & 300 &  90     & 2550 & 1400  &  186 & 5.62\\
L1165              & 300 &  135, 97\tablenotemark{b}     & 1500 & 660   &  57  & 3.90\\

\enddata
\tablecomments{} 
\tablenotetext{a}{Gradients are measured from center of the core as the protostars are located
at the edge.}
\tablenotetext{b}{Position axis for interferometer is slightly difference to capture the most kinematic
detail.}
\end{deluxetable}


==> tab4.tex <==
\begin{deluxetable}{llllll}

\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Source Properties}
\tablehead{
  \colhead{Source} & \colhead{Distance} & \colhead{N2H+/N2D+ offset}  & \colhead{$R_{SS}$} & \colhead{$R_C$(9000)} & \colhead{$R_C$(R_{SS})}& \colhead{Gradient (9000)\\
                    & \colhead{pc}      & \colhead{($^{\prime\prime}$)}  & \colhead{(AU)} & \colhead{(AU)} & \colhead{(AU)} & \colhead{(km s$^{-1}$ pc$^{-1}$)} \\

}
\startdata
IRAS 03282+3035    & 300 & 8   & -    & -     &  -   & -   \\
HH211-mm           & 300 & 0   & 1000?& 7100  &  2   & 12.83\\
L1521F             & 140 & 0   & -    & 20    &  -   & 0.68\\
IRAS 04325+2402    & 140 & 0   & -    & -     &  -   & 6.89\tablenotemark{\dagger}\\
L1527              & 140 & 40  & 1120 & 1600  &  11  & 6.01\\
RNO43              & 420 & 15  & 1800 & 1500  &  230 & 5.84\\
HH270 VLA1         & 420 & N/A & -    & -     &  -   & -   \\
IRAS 16253-2429    & 125 & N/A & 1300 &  3    &  -   & 0.62\\
L483               & 200 & 18  & -    & 2150  &  -   & 7.05\\
Serpens MMS3       & 300 & N/A & 1800 & 430   &  85  & 3.15\\
HH108IRS           & 300 & 0   & 1950 & 140   &  43  & 1.8 \\
L673-SMM2          & 300 & 22  & -    & -     &  -   & -   \\
L1152              & 300 & 10  & -    & -     &  -   & 3.27\tablenotemark{\dagger}\\
L1157              & 300 & 15  & 1350 & 150   &  14  & 1.86\\
CB230              & 300 & N/A & 2550 & 1400  &  186 & 5.62\\
L1165              & 300 & 15  & 1500 & 660   &  57  & 3.90\\

\enddata
\tablecomments{} 
\tablenotetext{\dagger}{Gradients are measured from center of the core as the protostars are located
at the edge.}
\end{deluxetable}

